Multi-tier Automated Planning for Adaptive Behavior (Extended Version)

A planning domain, as any model, is never complete and inevitably makes assumptions on the environment's dynamic. By allowing the specification of just one domain model, the knowledge engineer is only able to make one set of assumptions, and to specify a single objective-goal. Borrowing from work in Software Engineering, we propose a multi-tier framework for planning that allows the specification of different sets of assumptions, and of different corresponding objectives. The framework aims to support the synthesis of adaptive behavior so as to mitigate the intrinsic risk in any planning modeling task. After defining the multi-tier planning task and its solution concept, we show how to solve problem instances by a succinct compilation to a form of non-deterministic planning. In doing so, our technique justifies the applicability of planning with both fair and unfair actions, and the need for more efforts in developing planning systems supporting dual fairness assumptions.

==> fig-example-controller.tex <==
\begin{tikzpicture}[node distance=2cm]

    \tikzstyle{every node}=[draw, ellipse, inner sep=0pt, align=center,shape border rotate=90]
        \node[initial,state,ellipse,inner sep=0pt]            				(q0)      
        {\pddl{act} \\
         \pddl{at(c2)} \\
         \pddl{-scratch} \\
         \pddl{-u_walk} \\
         \pddl{l3}
            };
    \node[state,right of=q0,xshift=3cm]  			(q1)      {$n_1$};
    \node[state,below left of=q1,xshift=-1cm]     (q2)      {$n_2$};
      
    \path (q0) edge[bend left=15]        			node[]  	{\pddl{(at agent work)}}         (q1);
    \path (q1) edge[bend left=0]       node[]  
            {\begin{tabular}{c}
                \pddl{(at agent home)}\\
                \pddl{(at car home)}
            \end{tabular}}         
            (q0);
    \path (q1) edge[bend left]        node[xshift=-.5cm] 	
            {$\pddl{(at agent pub)}$}         (q2);
    \path (q2) edge[bend left]     	node[xshift=.8cm]  	
          {\begin{tabular}{c}
                \pddl{(at agent home)}\\
                \pddl{(at car home)}
            \end{tabular}}         
            (q0);
    \path (q2) edge[loop below]                 node[]  	{$\pddl{(had agent drinks)}$}         (q3);
  \end{tikzpicture}
